Chip-Surface Based Visual Authentication for Integrated Circuits

The rapid development of the semiconductor industry and the ubiquity of electronic devices have led to a significant increase in the counterfeiting of integrated circuits (ICs). This poses a major threat to public health, the banking industry, and military defense sectors that are heavily reliant on electronic systems. The electronic physically unclonable functions (PUFs) are widely used to authenticate IC chips at the unit level. However, electronic PUFs are limited by their requirement for IC chips to be in working status for measurements and their sensitivity to environmental variations. This paper proposes using optical PUFs for IC chip authentication by leveraging the unique microscopic structures of the packaging surface of individual IC chips. The proposed method relies on color images of IC chip surfaces acquired using a flatbed scanner or mobile camera. Our initial study reveals that these consumer-grade imaging devices can capture meaningful physical features from IC chip surfaces. We then propose an efficient, lightweight verification scheme leveraging specular-reflection-based features extracted from videos, achieving an equal error rate (EER) of 0.0008. We conducted factor, sensitivity, and ablation studies to understand the detailed characteristics of the proposed lightweight verification scheme. Our work is the first to apply the optical PUF principle for the authentication of IC chips, synergizing image and video processing with semiconductor chip technology and demonstrating the potential to significantly enhance the security of the semiconductor supply chain.

==> tex_figs/fig_impact_eer_vs_frame_count.tex <==
\begin{figure}[!t]
\centering
  \vspace{-1mm}
  \hspace{-1mm}
  \subfloat[]{\includegraphics[width=0.48\linewidth]{figs/correlations_num_frames.eps}}
  \subfloat[]{\includegraphics[width=0.48\linewidth]{figs/correlations_num_frames_lap.eps}}
	\caption{The impact of number of frames sampled per video to calculate correlations on the authentication performance: EER against the number of frames when assuming (a) Gaussian and (b) Laplace distributions. More sampled frames will result in a smaller EER.}
  \label{fig:correlation_frame_num}
\end{figure}
